Optimizing Data Usage via Differentiable Rewards

To acquire a new skill, humans learn better and faster if a tutor, based on their current knowledge level, informs them of how much attention they should pay to particular content or practice problems. Similarly, a machine learning model could potentially be trained better with a scorer that "adapts" to its current learning state and estimates the importance of each training data instance. Training such an adaptive scorer efficiently is a challenging problem; in order to precisely quantify the effect of a data instance at a given time during the training, it is typically necessary to first complete the entire training process. To efficiently optimize data usage, we propose a reinforcement learning approach called Differentiable Data Selection (DDS). In DDS, we formulate a scorer network as a learnable function of the training data, which can be efficiently updated along with the main model being trained. Specifically, DDS updates the scorer with an intuitive reward signal: it should up-weigh the data that has a similar gradient with a dev set upon which we would finally like to perform well. Without significant computing overhead, DDS delivers strong and consistent improvements over several strong baselines on two very different tasks of machine translation and image classification.

==> abstract.tex <==
\begin{abstract}
Good training data matters. While deep learning models in general benefit from a large amount of training data, low-quality training data such as noisy, out-of-domain, or adversarial data are detrimental to the learning of these models. Meanwhile, identifying the optimal set of training instances is a challenging problem, since the effect of any given set of data usually only becomes visible at the end of the training, which is a long and expensive process. In this paper, we propose Differentiable Data Selection~(\dds), a novel method for selecting high-quality training data. The selection process is parameterized as a differentiable function, which can be efficiently trained along with the model that consumes the selected data. On two modalities, we show that without significant computing overhead, \dds~delivers strong and consistent improvements. Specifically, on multilingual machine translation, \dds~can identify which related languages are helpful to improve the translation of another language, leading to consistent improvements over a strong heuristic data selection baseline. On image classification tasks with CIFAR-10 and ImageNet, and with different ranges of data, \dds~can also identify the importance of the training instance, leading to consistent improvements over the baselines in all settings. Code will be available up on acceptance.\footnote{If our paper is accepted, but we do not submit our code along with the camera-ready version, we will courteously retract the accepted paper.}

\end{abstract}

==> algorithm.tex <==
\section{\label{sec:alg}Algorithm}

\begin{algorithm}[H]
\SetAlgoLined
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetCommentSty{itshape}
\SetKwComment{Comment}{$\triangleright$\ }{}
%\KwResult{Write here the result }
\Input{Multilingual Corpus C, with $n$ source languages $(S_1, S_2,...,S_n)$}
\Output{The converged NMT model $\theta^*$}
 Initialize the agent $g(i|x, y; \omega)$, and the NMT model $\theta$
 
 \While{$\theta$ not converged}{
  X, Y = load\_data(g(x, y; \omega), C)
  
  optimize\_NMT(\theta, X, Y)
  
  grad\_vec = calculate\_grad\_prod($S$, $S_1, S_2, ..., S_n$)
  
  \For{ iter in E}{
  
    sample $B$ data pairs from $C$
  
    optimize $g$ by minimizing the loss 
  $-\frac{1}{B} \sum_{j=1}^B \sum_{i=1}^n \text{grad\_vec}[i] \cdot \text{log}(g(i|x_j, y_j;\omega))$ 
  }
  
  
 }
 \caption{Training multilingual NMT data selection agent}
\end{algorithm}

%\begin{algorithm}[h]
%  \caption{The first method of making balanced binary tree}
%  \small
%  \DontPrintSemicolon
%  \SetKwInOut{Input}{Input}
%  \SetCommentSty{itshape}
%  \SetKwComment{Comment}{$\triangleright$\ }{}
%  % \SetAlgoNoEnd
%  % \SetAlgoNoLine
%  \SetKwInOut{Output}{Output}
%  \SetKwFunction{FMakeTree}{make\_tree\_v1}
%  \SetKwProg{Fn}{Function}{:}{}
%  \Input{$w$: the list of words in a sentence, $l$: start index, $r$: end index}
%  \Output{a balanced binary tree for words from $l$ to $r$ in $w$}
%  \Fn{\FMakeTree{$w$, $l$, $r$}}{
%  %  \If {$l = r$} { 
%  %    \KwRet $\textrm{TerminalNode}(w[l])$\;
%  %  }
%  %  \;
%  %  $m = \text{floor}((l + r) / 2)$ \Comment*[r]{index of split point} 
%  %  $\textit{left\_tree} = \textrm{make\_tree\_v1}(w, l, m)$ \;
%  %  $\textit{right\_tree}= \textrm{make\_tree\_v1}(w, m+1, r)$ \;
%  %  \;
%  %  \KwRet $\textrm{NonTerminalNode}(\textit{left\_tree}, \textit{right\_tree})$
%  }
%\end{algorithm}

==> introduction.tex <==
\section{\label{sec:intro} Introduction}

While deep learning models are remarkably good at fitting large data sets, they are also highly sensitive to the quality, or even structural or domain properties of the data with which they are provided.
Prior work has found that removing noisy data, or selecting in-domain or structurally similar data can lead to large improvements in model performance while potentially reducing the training time~\citep{jiang-zhai-2007-instance,wang-etal-2017-instance,axelrod2011domain,foster-etal-2010-discriminative,moore2010intelligent}. Most of the existing data selection methods involve heuristics designed through domain-specific knowledge, which are difficult to generalize across tasks and have no guarantees of optimality.
In this paper, we ask the question: ``can we design an algorithm that automatically and efficiently learn the optimal training data for any given learning model?''

We propose a general algorithmic framework for automatic data selection that works by optimizing a data scoring function throughout the training process. We formulate the training objective of the model itself as a weighted sum of the \textit{training} loss using a scoring function. We then optimize this scoring function so that the learned model parameters minimize the loss on the \textit{development} set. The solution of this mathematical formulation leads to a simple optimization rule for the data scoring function: it should upweight the training instances that have similar gradients with the gradients of the development data. We name this method ``Differentiable Data Selection~(\dds)'', because the update rule allows us to directly optimize the data scoring function using back-propagation. 

We demonstrate two concrete instantiations of the \dds~framework, one for a more general case of image classification, and the other for a more specific use case on neural machine translation~(NMT). For image classification, we test the algorithm on both CIFAR-10 and ImageNet. For NMT, we focus on a multilingual setting, where we select data from a multilingual corpus to improve the performance on a particular language. 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method.tex <==
\section{\label{sec:method}Differentiable Data Selection}
\subsection{\label{sec:dds_motivation}Motivation}

% \gn{I made a number of suggestions below based on the fact that it's not just $\ell_{\text{train}}$ and $\ell_{\text{dev}}$ that changed, but also $\mathcal{D}_{\text{train}}$ and $\mathcal{D}_{\text{dev}}$. An alternative would be to define $J_{\text{train}}(\theta)$ and  $J_{\text{dev}}(\theta)$, which are based on the training data and development data, then discuss the fact that you're trying to close the gap between the two.}
% \gn{I also think it might not be immediately obvious to many people why $\ell_{\text{train}}$ and $\ell_{\text{dev}}$ may be different? From the description here (n.b., I haven't read beyond Section 2.1 while writing this comment, which I think is fine because people read papers linearly), I would guess you mean something like $\ell_{\text{train}}$ is an efficient-to-compute maximum likelihood objective and $\ell_{\text{dev}}$ is a slow-to-compute RL or minimum risk objective?}
% \gn{I think describing Section 2.1 super-clearly is important here. This is an exciting idea, and I think if we explain it well people will be excited about it! Let's polish this section a lot.}
% \gn{One idea: what about making $J(\theta)$ itself be parameterized by a loss function and a data distribution? Then we can plug in any loss and data that we prefer later without re-defining equations?}
% \an{Another idea (that I am ambivalent about): After section 2.2, you drop $(x,y)$ from the notation. I associate (x,y) with single input/output, which is not necessarily the case. Maaaaybe substitute all $(x,y)$ with $d$ e.g. $\ell_{\text{dev}}(d;\theta)$ and $d \sim \text{Uniform}(\mathcal{D}_{\text{train}})$?}

Commonly in machine learning, we seek to find parameters $\theta$ that minimize the \emph{risk} $J(\theta,P)$, the expected value of a loss function $\ell(x, y; \theta)$,
%\paul{AKA empirical risk if you want to pander to ML savvy reviewers} \gn{actually, not ``empirical risk'', just ``risk'', unless we're defining it over a particular set of data. But good point though. I've modified the explanation.}
where $\langle x, y \rangle$ are pairs of inputs and associated labels sampled from a particular distribution $P(X, Y)$:
\begin{equation}
  \label{eqn:generic_optim}
   \small
  \begin{aligned}
    \theta^* = \argmin_\theta J(\theta, P)
    ~~~\text{where}~~~
    J(\theta, P) = \mathbb{E}_{x, y \sim P(X, Y)} [\ell(x, y; \theta)]
  \end{aligned}
\end{equation}

In the ideal case, we would like the risk $J(\cdot)$ to be minimized over the inputs and outputs that we will expect our system to see at test time, defined as $P_{\text{test}}(X,Y)$.
Unfortunately, this distribution is unknown at training time, so instead we collect a training set $\mathcal{D}_\text{train} = \{(x_i, y_i): i = 1, ..., N_\text{train}\}$ with distribution $P_\text{train}(X, Y)$, and minimize the \emph{empirical risk} by taking $\langle x, y \rangle \sim \text{Uniform}(\mathcal{D}_\text{train})$.
Since we need a large enough $\mathcal{D}_\text{train}$ to train a good model, it is hard to ensure that $P_\text{train}(X, Y) \approx P_{\text{test}}(X, Y)$, and in fact one frequently has to be content with training data from a very different distribution than what we see at test time.
However, it is generally possible to collect a relatively small development set $\mathcal{D}_\text{dev}= \{(x_i, y_i): i = 1, ..., N_\text{dev}\}$ with distribution $P_{\text{dev}}(X, Y) \approx P_{\text{test}}(X, Y)$.
The discrepancy between $P_\text{train}(X, Y)$ and $P_\text{dev}(X, Y)$ manifests itself in the form of problems such as overfitting~\citep{overfit_random_examples,dropout}, covariate shift~\citep{shimodaira2000improving}, and label shift~\citep{lipton2018detecting}.
%exposure bias~\citep{dad_nmt,mixer_nmt} \gn{I'm not sure that this is a good example, as I think exposure bias is maybe a bigger feature of the loss function $\ell$ than the data mismatch? What about instead talking about ``co-variate shift'' and ``label shift'', e.g. \cite{lipton2018detecting}?}.
Since we can assume that the data in $\mathcal{D}_\text{dev}$ is a better approximation of our test-time scenario, we argue that it is possible, and reasonable to use $\mathcal{D}_\text{dev}$ to inform a better strategy for utilizing our available data in $\mathcal{D}_\text{train}$.

%We identify two issues with such formulation. First, while we seek a $\theta^*$, that minimizes $J(\theta)$ as in Eqn~\ref{eqn:generic_optim}, we evaluate $\theta^*$ on a development set $\mathcal{D}_\text{dev} = \{(x_i, y_i): i = 1, ..., N_\text{dev}\}$. While the distribution $P(X, Y)$ is unknown, in practice we can collect a relatively small development set $\mathcal{D}_\text{dev}$ with distribution $P_{\text{dev}}(X, Y) \approx P(X, Y)$.  The discrepancy between $P_\text{train}(X, Y)$ and $P_\text{dev}(X, Y)$ leads to various problems such as overfitting~\citep{overfit_random_examples,dropout} \paul{Overfitting is a property of the model, not the data. You can overfit a model on very good data} and exposure bias~\citep{dad_nmt,mixer_nmt}.\paul{So basically the point that this paragraph is trying to make is that the dev set has better quality and we should use that to inform our selection of training data right?}\cw{that's right}\paul{MAybe this could be made more explicit at the beginning of the paragraph. I'm not a fan of the first, [..], second construction here. How about: "in practice, it's hard to get good data in great quantity, [..]" and then explain the difference between train/dev.}

% \an{The `we' in this paragraph is not the same as the `we' in the next paragraph. I think we shouldn't use `we' in the first one. Maybe `one' or a scientist... `she'}

Specifically, we propose to replace the distribution $\text{Uniform}(\mathcal{D}_\text{train})$, with a parameterized distribution $p(X, Y; \psi)$ with support of $\mathcal{D}_\text{train}$ that brings the sampled data closer to $P_\text{dev}(X, Y)$ than when selected using the uniform distribution. In particular, data will be sampled by $\langle x, y \rangle \sim p(X, Y; \psi)$, 
and $\psi$ will be chosen so that $\theta^*$ that optimizes $J(\theta, p(X, Y;\psi))$ will approximately minimize $J(\theta, P_\text{dev}(X,Y))$: 
%\gn{A little pedantic, but $\psi$ isn't included anywhere in Eqn~\ref{eqn:generic_optim}. I think one easy way to fix this is instead of having $P(X,Y)$ be the true data distribution (unknown), you could have it be ``an arbitrary distribution''. Then you could say that ``ideally, this would match the true data distribution, but unfortunately this is not known''} 
\begin{equation}
  \label{eqn:psi_theta_argmin}
   \small
  \begin{aligned}
    \psi^* = \argmin_\psi
    \sum_{i=1}^{N_\text{dev}} \ell(x_i, y_i; \theta^*(\psi))
    ~\text{where}~
    \theta^*(\psi) = \argmin_\theta \mathbb{E}_{x, y \sim p(X, Y; \psi)} \left[ \ell(x, y; \theta) \right]
  \end{aligned}
\end{equation}
Directly optimizing for $\psi^*$ as above is prohibitively expensive, since finding $\argmin_\theta J(\theta)$ is by itself an expensive process, \eg~training a large neural network on a large dataset. 
Thus, we establish a mathematical formulation, which allows $\theta$ and $\psi$ to both be trained by stochastic gradient updates. As our method trains a differentiable distribution $p(X, Y; \psi)$ to select training data, we name the method \textit{Differentiable Data Selection}~(\dds).

\subsection{\label{sec:diff_data_selection}Framework}
For the rest of the section, we abbreviate the training objective $J(\theta, p(X, Y;\psi))$ as $J(\theta, \psi)$ for ease of notation. Similarly, we abbreviate the risk $J(\theta, \text{Uniform}(\mathcal{D}))$ over a dataset $\mathcal{D}$ as $J(\theta, \mathcal{D})$.

For a fixed value of $\psi$, $J(\theta, \psi)$ can be optimized using a stochastic gradient update. Specifically, at time step $t$, we update
\begin{equation}
  \label{eqn:theta_update_rule}
   \small
  \begin{aligned}
    \theta_t \leftarrow \theta_{t-1} - g\big( \nabla_\theta J(\theta_{t-1}, \psi) \big)
  \end{aligned}
\end{equation}
where $g(\cdot)$ is any function that may be applied to the gradient $\nabla_\theta J(\theta_{t-1}, \psi)$. For instance, in standard gradient descent $g(\cdot)$ is simply a linear scaling of $\nabla_\theta J(\theta_{t-1}, \psi)$ by a learning rate $\eta_t$, while with the Adam optimizer~\citep{adam} $g$ also modifies the learning rate on a parameter-by-parameter basis.

We now analyze how a gradient update as in Eqn~\ref{eqn:theta_update_rule} affects $J(\theta_t, \mathcal{D}_{\text{dev}})$. 
%\gn{Here, and in all following mentions, I think this should be $J(\theta, \mathcal{D}_{\text{dev}})$?}. \cw{eqn \ref{eqn:two_step_update} operates on $\ell(\mathbb{D}_\text{dev})$ so maybe it's easier to just use this?}
%\gn{Do we even need the following sentence? We're already calculating the gradient in Eqn~\ref{eqn:theta_update_rule}, so if we've already assumed $J(\cdot)$ is differentiable there, we can probably assume so here as well.} \cw{It might be worth it to mention it here, since eqn\ref{eqn:theta_update_rule} does not mention $\ell(\mathbb{D}_\text{dev})$} 
%\gn{Sometimes you're using $\theta_t$ and sometimes $\theta$. I'd be consistent (always use $\theta_t$)?} %To achieve this, we assume that $\ell(\mathcal{D}_\text{dev}; \theta_t)$ is differentiable with respect to $\theta_t$. This is not an unreasonable assumption,~\eg~log-likelihood objectives generally used in most neural prediction models are usually differentiable with respect to $\theta_t$. 
Due to the relationship between $\theta_t$ and $\psi$ as in Eqn~\ref{eqn:theta_update_rule}, $J(\theta_t, \mathcal{D}_\text{dev})$ is differentiable with respect to $\psi$. 
%Since evaluating  $J(\theta_t, \mathcal{D}_\text{dev})$ only requires $\theta_t$ and not $\psi$, 
By the chain rule, we can compute the gradient $\nabla_\psi J(\theta_t, \mathcal{D}_\text{dev})$ as follows:
%\gn{The first line here was actually pretty hard to follow for me. I think $\nabla J(\theta_t, \mathcal{D}_\text{dev})^\top$ should probably be $\nabla_{\theta_t} J(\theta_t, \mathcal{D}_\text{dev})^\top$, and $\nabla_\psi \theta_t(\psi)$ should be $\nabla_\psi \theta_t$ maybe? If so, please correct. Also maybe $J(\theta_{t-1})$ should be $J(\theta_{t-1}, \psi)$?}
\begin{equation}
  \label{eqn:two_step_update}
   \small
  \begin{aligned}
    \nabla_\psi J(\theta_t, \mathcal{D}_\text{dev})
      &= \nabla_{\theta_t} J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\psi \theta_t(\psi) &\text{(chain rule)} \\
      &= \nabla_{\theta_t} J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\psi \left( \theta_{t-1} - g\big( \nabla_\theta J(\theta_{t-1}) \big) \right) &\text{(substitute $\theta_t$ from Eqn~\ref{eqn:theta_update_rule})} \\
      &\approx -\nabla_{\theta_t} J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\psi g\big( \nabla_\theta J(\theta_{t-1}) \big) &\text{(assume $\nabla_\psi \theta_{t-1} \approx 0$)} %\paul{why? doesn't sound like this would be the case. More specifically either you have a reason to say $\partial \theta_{t-1} / \partial \psi = 0$(and not $\approx$) or you must justify this experimentally.})}
  \end{aligned}
\end{equation}
Here, we make a Markov assumption that $\nabla_\psi \theta_{t-1} \approx 0$, assuming that at step $t$, given $\theta_{t-1}$ we do not care about how the values of $\psi$ from previous steps led to $\theta_{t-1}$. Eqn~\ref{eqn:two_step_update} leads to a rule to update $\psi$ using gradient descent:
\begin{equation}
  \label{eqn:psi_update_rule}
   \small
  \begin{aligned}
    \psi_{t+1} 
      &\leftarrow \psi_t + \eta_\psi \nabla_{\theta_t} J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\psi g\big( \nabla_\theta J(\theta_{t-1}, \psi_t) \big),
  \end{aligned}
\end{equation}
where $\eta_\psi$ is the learning rate for $\psi$, which is a hyper-parameter. Note that Eqn \ref{eqn:psi_update_rule} involves a calculation of the nested gradient, which is similar to some ideas in prior work on optimization~\citep{hyper_grad}, meta-learning~\citep{finn2017model}, and neural architecture search~\citep{darts}. 
%\gn{haha, a little more detail might be warranted here :) ``prior work on XXX (cite), YYY (cite), and ZZZ (cite)}. 
However, we are the first to utilize the idea for data selection to reduce discrepancy between the training and dev sets. 

One reasonable concern that may be raised with this approach is that because we optimize $\psi_t$ directly on the dev set using $J(\theta_t, \mathcal{D}_\text{dev})$, we may risk indirectly overfitting model parameters $\theta_t$ by selecting a small subset of data that is overly specialized.
However we do not observe this problem in practice, and posit that this because (1) the influence of $\psi_t$ on the final model parameters $\theta_t$ is quite indirect, and acts as a ``bottleneck'' which has similarly proven useful for preventing overfitting in neural models \cite{grezl2007probabilistic}, and (2) because the actual implementations of DDS~(which we further discuss in Section \ref{sec:formualtion}) only samples a subset of data from $\mathcal{D}_\text{train}$ at each optimization step, further limiting expressivity.
%\gn{Let me revive Paul's comment here: I think this is an important discussion (I believe I also brought this up when speaking with Cindy, independently of Paul, so this is definitely something people paying attention will notice). Let's try to add this somewhere, perhaps at the end of this section.}
%\paul{One central comment here: one could argue that if your goal is to minimize $\ell_\text{dev}(\theta)$ you could just do gradient descent on the dev set (which is bad of course), furthermore under mild conditions \footnote{if $\ell_{\text{dev}}$ is within the linear span of all $\ell_{\text{train}}$ which is the case if $N>d$ and the gradients are linearly independent, and provided $p(\ldots;\psi)$ is sufficently expressive} it is in theory possible that you learn $\psi$ such that $\nabla J = \nabla \ell_{\text{dev}}$ . Therefore there needs to be some kind of regularization on $\psi$ such that this is not the case. Obviously your experimental result show that there is some kind of implicit regularization in your choice of model for $p(\ldots ; \psi)$ but it would be better to formulate this more explicitly, because this is for sure something that a reviewer might point out.}

\dds~operates by alternating Eqn~\ref{eqn:theta_update_rule} and Eqn~\ref{eqn:psi_update_rule} on batches of training data and dev data respectively. To implement Eqn~\ref{eqn:psi_update_rule} we need two approximations.
First, in practice the size of $\mathcal{D}_\text{train}$ is usually too large for exact calculation of the gradient $\nabla_\theta$. To overcome this difficulty, we adopt an importance sampling strategy, which can be implemented in two ways:
(1) We can sample a subset of $\mathcal{D}_{\text{train}}$ with a uniform proposal distribution $\hat{x}, \hat{y} \sim \text{Uniform}(\mathcal{D}_\text{train})$, then scale the probabilities in Eqn~\ref{eqn:psi_theta_argmin} by $p(\hat{x}, \hat{y}; \psi)$ over only this subset of data.
(2) We can similarly sample a subset of $\mathcal{D}_{\text{train}}$ uniformly, but then take a Monte-Carlo estimate of this quantity by further sub-sampling the data according to $p(\hat{x}, \hat{y}; \psi)$.
Second, we need to calculate the gradient $\nabla_\psi g$. This step depends on the optimization algorithm that we use for $\theta$, and we discuss some concrete formulations in the next section.

\section{\label{sec:grad_of_optimizers}Deriving $\nabla_\psi g$ for Different Optimizers}
%\gn{It seems reasonable to have this as a top-level section, so I changed it accordingly this has started to get into details that are probably better to separate from the overall high-level idea of DDS.}

Here we first derive $\nabla_\psi g$ for the general stochastic gradient descent~(SGD) update, then provide examples for two other common optimization algorithms, namely Momentum~\citep{nesterov} and Adam~\citep{adam}.
%\gn{It's not clear to me why you skip standard SGD without momentum? It seems like it'd make the most sense to start there, even if that's not what you finally use in experiments. If you use it in experiments then you definitely need to discuss it. Then when you explain momentum you could just point out the differences.}

\paragraph{SGD Updates.} The SGD update rule for $\theta$ is as follows
\begin{equation}
  \label{eqn:sgd_update}
   \small
  \begin{aligned}
    \theta_t &\leftarrow \theta_{t-1} - \eta_t \nabla_\theta J(\theta_{t-1}, \psi)
  \end{aligned}
\end{equation}
where $\eta_t$ is the learning rate. Matching the updates in Eqn~\ref{eqn:sgd_update} with the generic framework in Eqn~\ref{eqn:theta_update_rule}, we can see that $g$ in Eqn~\ref{eqn:theta_update_rule} has the form: %\gn{$J(\theta_{t-1})$ should be $J(\theta_{t-1}, \psi)$? There seem to be a few of these inconsistencies below as well, so please check. Also, which time step of $\theta$ does the gradient depend on?}
\begin{equation}
  \label{eqn:momentum_update_g}
   \small
  \begin{aligned}
    g\big(\nabla_\theta J(\theta_{t-1}, \psi)\big) = \eta_t \nabla_\theta J(\theta_{t-1}, \psi)
  \end{aligned}
\end{equation}
This reveals a linear dependency of $g$ on $\nabla_\theta J(\theta_{t-1, \psi})$, allowing the exact differentiation of $g$ with respect to $\psi$. From Eqn~\ref{eqn:psi_update_rule}, we have
\begin{equation}
  \label{eqn:momentum_update_for_psi}
   \small
  \begin{aligned}
    &\nabla J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\psi g\big( \nabla_\theta J(\theta_{t-1}, \psi) \big) \\
    &= \eta_t \cdot \nabla_\psi \mathbb{E}_{x, y \sim p(X, Y; \psi)} \left[J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\theta \ell(x, y; \theta_{t-1} )\right] \\
    &= \eta_t \mathbb{E}_{x, y \sim p(X, Y; \psi)} \left[\left( J(\theta_t, \mathcal{D}_\text{dev})^\top \cdot \nabla_\theta \ell(x, y; \theta_{t-1} ) \right) \cdot \nabla_\psi \log{p(x, y; \psi)} \right]
  \end{aligned}
\end{equation}
%\gn{This last paragraph was too dense for me to follow: could you please try to explain a little more?}
Here, the last equation follows from the log-derivative trick in the REINFORCE algorithm~\citep{reinforce}. 
%and can be implemented by Monte Carlo approximation.
%\gn{again, a little more detail here would be useful}. 
%Note we do not do reinforcement learning in this paper. Instead \gn{this ``instead'' was also not clear to me.}, we simply utilize the same log-derivative trick to compute $\nabla_\psi J(\theta_t, \mathcal{D}_\text{dev})$. 

\paragraph{Momentum Updates.} The momentum update rule for $\theta$ is as follows
\begin{equation}
  \label{eqn:momentum_update}
   \small
  \begin{aligned}
    m_t &\leftarrow \mu_t m_{t-1} + \eta_t \nabla_\theta J(\theta_{t-1}, \psi) \\
    \theta_t &\leftarrow \theta_{t-1} - m_t,
  \end{aligned}
\end{equation}
where $\mu_t$ is the momentum coefficient and $\eta_t$ is the learning rate. This means that $g$ has the form:
\begin{equation}
  \label{eqn:momentum_update_g}
   \small
  \begin{aligned}
    g(x) &= \mu m_{t-1} + \eta_t x \\
    g'(x) &= \eta_t
  \end{aligned}
\end{equation}
Therefore, the computation of the gradient $\nabla_{\psi}$ for the Momentum update is exactly the same with the standard SGD update rule in Eqn \ref{eqn:momentum_update_for_psi}.
%This reveals a linear dependency of $g$ on $\nabla_\theta J(\theta_{t-1})$, allowing the exact differentiation of $g$ with respect to $\psi$. From Eqn~\ref{eqn:psi_update_rule}, we have
%\begin{equation}
%  \label{eqn:momentum_update_for_psi}
%  \begin{aligned}
%    &\nabla \ell(\mathcal{D}_\text{dev}, \theta_t)^\top \cdot \nabla_\psi g\big( \nabla_\theta J(\theta_{t-1}, \psi) \big) \\
%    &= \eta_t \cdot \nabla_\psi \mathbb{E}_{x, y \sim p(X, Y; \psi)} \left[\ell(\mathcal{D}_\text{dev}, \theta_t)^\top \cdot \nabla_\theta \ell(x, y; \theta_{t-1} )\right] \\
%    &= \eta_t \mathbb{E}_{x, y \sim p(X, Y; \psi)} \left[\left( \ell(\mathcal{D}_\text{dev}, \theta_t)^\top \cdot \nabla_\theta \ell(x, y; \theta_{t-1} ) \right) \cdot \nabla_\psi \log{p(x, y; \psi)} \right]
%  \end{aligned}
%\end{equation}
%Here, the last equation is follows the log-derivative trick~\citep{reinforce}, and can be implemented by Monte Carlo approximation. Note we do not do reinforcement learning in this paper. Instead, we simply utilize the same log-derivative trick to compute $\nabla_\psi \ell(\mathcal{D}_\text{dev})$. 

\paragraph{Adam Updates.} We use a slightly modified update rule based on Adam~\citep{adam}:
\begin{equation}
  \label{eqn:adam_update}
   \small
  \begin{aligned}
    &g_t \leftarrow \nabla_\theta J(\theta_{t-1}, \psi) \\
    &v_t \leftarrow \beta_2 v_{t-1} + (1 - \beta_2) g_t^2 \\
    &\hat{v}_t \leftarrow v_t / (1 - \beta_2^t) \\
    &\theta_t \leftarrow \theta_{t-1} - \eta_t \cdot g_t / \sqrt{\hat{v}_t + \epsilon}
  \end{aligned}
\end{equation}
where $\beta_2$ and $\eta_t$ are hyper-parameters. This means that $g$ is a component-wise operation of the form:
\begin{equation}
  \label{eqn:adam_update_g}
   \small
  \begin{aligned}
    g(x) &= \frac{\eta_t \sqrt{1 - \beta_2^t} \cdot x}{\sqrt{\beta_2 v_{t-1} + (1 - \beta_2) x^2 + \epsilon}} \\
    g'(x) &= \frac{\eta_t \sqrt{1 - \beta_2^t} (\beta_2 v_{t-1} + \epsilon)}{\big( \beta_2 v_{t-1} + (1 - \beta_2) x^2 + \epsilon \big)^{3/2}} \approx \eta_t \sqrt{\frac{1 - \beta_2^t}{\beta_2 v_{t-1}}},  
  \end{aligned}
\end{equation}
%\paul{So all of this is under the assumption that $v_{t-1}$ is independent on $\psi$ right? maybe bring it up?}
the last equation holds because we assume $v_{t-1}$ is independent of $\psi$. Here the approximation makes sense because we empirically observe that the individual values of the gradient vector $\nabla_\theta J(\theta_{t-1}, \psi)$,~\ie~$g_t$, are close to $0$. Furthermore, for Adam, we usually use $\beta_2 = 0.999$. Thus, the value $(1 - \beta_2) x^2$ in the denominator of Eqn~\ref{eqn:adam_update_g} is negligible. With this approximation, the computation of the gradient $\nabla_\psi$ is almost the same with that for SGD in Eqn~\ref{eqn:momentum_update_for_psi}, with one extra component-wise scaling by the term in Eqn~\ref{eqn:adam_update_g}.

